Optimized parametric inference for the inner loop of the Multigrid Ensemble Kalman Filter

Essential features of the Multigrid Ensemble Kalman Filter (G. Moldovan, G. Lehnasch, L. Cordier, M. Meldi, A multigrid/ensemble Kalman filter strategy for assimilation of unsteady flows, Journal of Computational Physics 443-110481) recently proposed for Data Assimilation of fluid flows are investigated and assessed in this article. The analysis is focused on the improvement in performance due to the inner loop. In this step, data from solutions calculated on the higher resolution levels of the multigrid approach are used as surrogate observations to improve the model prediction on the coarsest levels of the grid. The latter represents the level of resolution used to run the ensemble members for global Data Assimilation. The method is tested over two classical one-dimensional problems, namely the linear advection problem and the Burgers' equation. The analyses encompass a number of different aspects, such as different grid resolutions. The results indicate that the contribution of the inner loop is essential in obtaining accurate flow reconstruction and global parametric optimization. These findings open exciting perspectives of application to grid-dependent reduced-order models extensively used in fluid mechanics applications for complex flows, such as Large Eddy Simulation (LES).

==> Cordier_Algorithm/Multigrid_EnKF_Moldovan.tex <==
% Version Moldovan original saved.
\begin{algorithm}
   \SetKw{init}{Initialization}
   \init$\Big\{\theta_{0}^{a,(i)},\big(x_{0}^F\big)^a, \big(x_{0}^C\big)^{a,(i)}\Big\}$ with $i=1,...,N$;\\% $k:=0$; $\theta_0 \sim \mathcal{N}(0, Q_\theta)$; $(u)^F(x,0)=u_0$; $(u^{(i)})^C(x,0)=u_0$;  $i=1,...,N$; $\Phi=\Phi_0$\\
   
   \While{$k<T$}{
	
	Fine grid forecast:
       $\big(x_k^{F}\big)^f=\mathcal{M}^F_{k:k-1}\Big(\big(x_{k-1}^{F}\big)^a,\overline{\theta}_{k}^a \Big)$;\\  %$u(0,t)=u_0+\overline{a} sin(\omega t)$\\
      Parameter error inflation: $\theta_k^{f,(i)}=\theta_{k-1}^{a,(i)}+\tau^{(i)}_k$, $\tau^{(i)}_k\sim\mathcal{N}(0,\Sigma^{\theta}_k)$\\
      
      Ensemble coarse forecast: $\big(x_k^C\big)^{f,(i)}=\mathcal{M}_{k:k-1}^{C}\Big(\big(x_{k-1}^C\big)^{a,(i)},\theta_{k}^{f,(i)}\Big)$;\\
     
      \If {Observation available}{
	  Creation of an ensemble of observations: $\big(y_k^C\big)^{o,(i)}=\big(y_k^C\big)^{o}+\big(\epsilon^C\big)^{o,(i)}$, $\big(\epsilon^C\big)^{o,(i)} \sim \mathcal{N}(0,R_k^C)$\\
	  Compute normalized anomalies with $\big(y^C_k\big)^{f,(i)}$=$\mathcal{H}_k^C\Big( \big(x^C_k\big)^{f,i}\Big)$:\\
	  $\Big[\Theta^f_k\Big]_{:,i}=\frac{\theta^{f,(i)}_k-\overline{\theta^f_k}}{\sqrt{N-1}}$; $\Big[Y^f_k \Big]_{:,i}=\frac{\big(y^C_k\big)^{f,(i)}-\big(\overline{y^C_k}\big)^f}{\sqrt{N-1}}$\\
      $\theta$ Kalman Gain: $\big(K^C_k\big)^{\theta,e}=\Theta^f_k \big(Y_k^f\big)^T(Y_k^f \big(Y_k^f\big)^T+R_k^C)^{-1}$\\
      $\theta$ correction:
      $\theta_k^{a,(i)}=\theta_k^{f,(i)}+\big(K_k^C\big)^{\theta,e}\Big[\big(y_k^C\big)^{o,(i)}-\big(y^C_k\big)^{f,(i)}\Big]$\\
      Ensemble coarse forecast: $\big(x_k^C\big)^{f,(i)}=\mathcal{M}_{k:k-1}^{C}\Big(\big(x_{k-1}^C\big)^{a,(i)},\theta_{k}^{a,(i)}\Big)$;\\
      Compute normalized anomalies with $\big(y^C_k\big)^{f,(i)}$=$\mathcal{H}_k^C\Big( \big(x^C_k\big)^{f,i}\Big)$:\\
	  $\Big[\big(X^C_k\big)^f \Big]_{:,i}=\frac{\big(x^C_k\big)^{f,(i)}-\big(\overline{x^C_k}\big)^f}{\sqrt{N-1}}$; $\Big[Y^f_k \Big]_{:,i}=\frac{\big(y^C_k\big)^{f,(i)}-\big(\overline{y^C_k}\big)^f}{\sqrt{N-1}}$\\
	  $x$ Kalman Gain: $\big(K_k^C\big)^{x,e}=\big(X_k^C\big)^f Y_k^T(Y_k Y_k^T+R_k^C)^{-1}$\\
      $x$ correction: $\big(x_k^C\big)^{a,(i)}=\big(x_k^C\big)^{f,(i)}+\big(K_k^C\big)^{x,e}\Big[\big(y_k^C\big)^{o,(i)}-\big(y^C_k\big)^{f,(i)}\Big]$
      
      
      

	  Projection on the coarse grid $\left(x^{C}_k\right)^{*}=\Pi^F_C\left(\left(x_k^{F}\right)^f\right)$;\\
	  Fine grid state corrected with the ensemble statistics:\\
	  $\left(x^{C}_k\right)^{'}=\left(x^{C}_k\right)^{*}+\left(K_k^C\right)^{x,e}\left[\left(y_k^{C}\right)^o-\mathcal{H}_k^C\left(\left(x_k^{C}\right)^{*}\right)\right]$;\\
	  $\left(x^{F}_k\right)^{'}=\left(x_k^{F}\right)^f+\Pi^C_F\left(\left(x^{C}_k\right)^{'}-\left(x^{C}_k\right)^{*}\right) $;\\ 

      Matrix-Splitting iterative procedure on the final solution starting from $x_k^0=\big(x^{F}_k\big)^{'}$. 
			%Relaxation factor $\alpha=0.5$ used to obtain $\left(x^F_k\right)^a$
			}
      %$\Psi_{k:k-1}^{'}u^a_k=\Psi_{k:k-1}u^{a}_{k-1}$, $\Psi_{k:k-1}=\Psi_{k:k-1}\big(u^{a}_{k-1},\overline{\theta}_{k-1}^a\big)$, $\Psi_{k:k-1}^{'}=\Psi_{k:k-1}^{'}\big(u^{'}_{k},\overline{\theta}_{k}^a\big)$ \\
 
      
            $k:=k+1$;\\
            
   }
   \caption{Multigrid EnKF algorithm.}
   \label{alg:algo_KF_corrected_corrected}
\end{algorithm}

==> Sec2-lo.tex <==
%\section{Model equations \& sequential state estimation}
\section{Ensemble Kalman Filter (EnKF) and multigrid version (MGEnKF)}
\label{sec:maths}

The Kalman Filter (KF) \cite{Kalman1960_jbe} is a sequential data assimilation tool which provides an estimation of a state variable at time $k$ ($\mathbf{x}_k$), combining the initial estimate $\mathbf{x}_0$, a set of observations $\mathbf{y}^\text{o}_k$, and a linear dynamical model $\mathbf{M}_{k:k-1}$. The state estimation is obtained via two successive operations, which are usually referred to as \textit{forecast} step (superscript $f$) and \textit{analysis} step (superscript $a$). The classical version of the algorithm reads as follows:

\begin{subequations}
\begin{align}
\mathbf{x}^\text{f}_{k} & = \mathbf{M}_{k:k-1} \mathbf{x}^\text{a}_{k-1}\label{eq:x_mdl_kf}\\
\mathbf{P}^\text{f}_{k}& = \mathbf{M}_{k:k-1} \mathbf{P}^\text{a}_{k-1} {\mathbf{M}^\top_{k:k-1}}+\mathbf{Q}_k \label{eq:P_mdl_kf} \\
  \mathbf{K}_k& = \mathbf{P}^\text{f}_{k}{\mathbf{H}^\top_k}\left(\mathbf{H}_k \mathbf{P}^\text{f}_{k} {\mathbf{H}^\top_k}+\mathbf{R}_k\right)^{-1}\label{eq:k_kf}\\
  \mathbf{x}^\text{a}_{k}& = \mathbf{x}^\text{f}_{k} + \mathbf{K}_k\left(\mathbf{y}^\text{o}_k-\mathbf{H}_k\mathbf{x}^\text{f}_{k}\right)\label{eq:x_kf}\\
  \mathbf{P}^\text{a}_{k}& = \left(I-\mathbf{K}_k \mathbf{H}_k\right)\mathbf{P}^\text{f}_{k}\label{eq:P_kf}
\end{align}
\end{subequations}

The final state estimation $\mathbf{x}^\text{a}_{k}$ is obtained in \eqref{eq:x_kf} by combining the predictor solution $\mathbf{x}^\text{f}_{k}$ and a correction term accounting for the real observation $\mathbf{y}^\text{o}_k$ and the observation predicted from $\mathbf{x}^\text{f}_{k}$ through the linear observation operator $\mathbf{H}_k$. This correction term is weighted by the matrix $\mathbf{K}_k$, usually referred to as \textit{Kalman gain}. The matrices $\mathbf{Q}_k$ and $\mathbf{R}_k$ measure the level of confidence in the model and in the observation, respectively. The error covariance matrix $\mathbf{P}^{\text{f}/\text{a}}_k$, defined as $
\mathbb{E}\left[
\left(\mathbf{x}_k^{\text{f}/\text{a}} - \mathbb{E}(\mathbf{x}_k^{\text{f}/\text{a}})\right) 
\left(\mathbf{x}_k^{\text{f}/\text{a}} - \mathbb{E}(\mathbf{x}_k^{\text{f}/\text{a}})\right)^\top \right]$, is advanced in time in the \textit{forecast} step \eqref{eq:P_mdl_kf} and manipulated in the \textit{analysis} step \eqref{eq:P_kf}.    

These last two operations are usually extremely expensive and they may require computational resources that are orders of magnitude larger than the model operation. In order to alleviate such computational issues, one possible alternative is to provide an approximation of $\mathbf{P}$ using stochastic Monte-Carlo sampling. The Ensemble Kalman Filter (EnKF) \cite{Evensen1994,Evensen2009_Springer} provides an approximation of $\mathbf{P}_k$ by means of an ensemble of $N_\text{e}$ states.

Given an ensemble of forecast/analysis states at a given instant $k$, the ensemble matrix collecting the information of the database is defined as:
\begin{equation}
\pmb{\mathscr{E}}_k^{\text{f}/\text{a}}=
\left[\mathbf{x}_k^{\text{f}/\text{a},(1)},\cdots,\mathbf{x}_k^{\text{f}/\text{a},(N_\text{e})}\right]\in\mathbb{R}^{N_x\times N_\text{e}} \label{eq:Ensemble_Matrix}
\end{equation}

Starting from the data assembled in $\pmb{\mathscr{E}}_k^{\text{f}/\text{a}}$, the ensemble mean 
%$\overline{\mathbf{x}_k^{\text{f}/\text{a}}}$
\begin{equation}
    \overline{\mathbf{x}_k^{\text{f}/\text{a}}}=\frac{1}{N_\text{e}}\sum^{N_\text{e}}_{i=1}\mathbf{x}_k^{\text{f}/\text{a},(i)} \label{eq:Ensemble_Mean}
\end{equation} 

is used to obtain the normalized ensemble anomaly matrix:
\begin{equation}
\mathbf{X}_k^{\text{f}/\text{a}}=\frac{\left[\mathbf{x}_k^{\text{f}/\text{a},(1)}-\overline{\mathbf{x}_k^{\text{f}/\text{a}}},\cdots,\mathbf{x}_k^{\text{f}/\text{a},(N_\text{e})}-\overline{\mathbf{x}_k^{\text{f}/\text{a}}}\right]}{\sqrt{N_\text{e}-1}}\in\mathbb{R}^{N_x\times N_\text{e}}, \label{eq:Ensemble_Anomaly}
\end{equation}


The approximated error covariance matrix, hereafter denoted with the superscript $e$,  is obtained via the matrix product: 
\begin{equation}
\mathbf{P}_k^{\text{f}/\text{a},\text{e}}=\mathbf{X}_k^{\text{f}/\text{a}} \left(\mathbf{X}_k^{\text{f}/\text{a}}\right)^\top\in\mathbb{R}^{N_x\times N_x} \label{eq:Ensemble_P}
\end{equation}

The goal of the EnKF is to mimic the BLUE (Best Linear Unbiased Estimator) analysis of the Kalman filter.
For this,  Burgers et al. \cite{Burgers1998} showed that the observation must be considered as a random variable with an average corresponding to the observed value and a covariance $\mathbf{R}_k$ (the so-called \emph{data randomization} trick).
Therefore, given the discrete observation vector $\mathbf{y}^\text{o}_k\in \mathbb{R}^{N_y}$ at an instant $k$, the ensemble of perturbed observations is defined as:
\begin{equation}
\mathbf{y}_k^{\text{o},(i)}=\mathbf{y}_k^\text{o}+\mathbf{\epsilon}_k^{\text{o},(i)},
\quad
\text{with}
\quad
i=1,\cdots,N_\text{e}
\quad
\text{and}
\quad
\mathbf{\epsilon}_k^{\text{o},(i)}\sim \mathcal{N}(0,\mathbf{R}_k)
.\label{eq:perturbed_y}
\end{equation}

%In a similar way to what we did for the ensemble matrices of the forecast/analysed states, we define
A normalized anomaly matrix of the observations errors is defined as
\begin{equation}
\mathbf{E}_k^{\text{o}}=
\frac{1}{\sqrt{N_\text{e}-1}}
\left[
\mathbf{\epsilon}_k^{\text{o},(1)}-\overline{\mathbf{\epsilon}_{k}^{\text{o}}},
\mathbf{\epsilon}_k^{\text{o},(2)}-\overline{\mathbf{\epsilon}_{k}^{\text{o}}},
\cdots,
\mathbf{\epsilon}_k^{\text{o},(N_\text{e})}-\overline{\mathbf{\epsilon}_{k}^{\text{o}}},
\right]
\in\mathbb{R}^{N_y\times N_\text{e}}
\end{equation} 
where
$\displaystyle\overline{\mathbf{\epsilon}_{k}^{\text{o}}}=\frac{1}{N_\text{e}}\sum_{i=1}^{N_\text{e}}\mathbf{\epsilon}_k^{\text{o},(i)}$.

The covariance matrix of the measurement error can then be estimated as
\begin{equation}
\mathbf{R}_k^\text{e}=\mathbf{E}^\text{o}_k \left(\mathbf{E}^\text{o}_k\right)^\top\in\mathbb{R}^{N_y\times N_y}. \label{eq:observation_matrix_errorcov}
\end{equation}

Combining the previous results, one obtains (see \cite{Asch2016_SIAM}) the standard stochastic EnKF algorithm. The corresponding analysis step consists of updates  performed on each of the ensemble members, as given by 
\begin{equation}
\mathbf{x}_k^{\text{a},(i)}=
\mathbf{x}_k^{\text{f},(i)}+
\mathbf{K}_k^\text{e}
\left(y_k^{\text{o},(i)}-\mathbf{\mathcal{H}}_k\left(\mathbf{x}^{\text{f},(i)}_k\right)\right)\label{eq:ensemble_update}
\end{equation}
where $\mathbf{\mathcal{H}}_k$ is the non-linear observation operator. The expression of the Kalman gain is
\begin{equation}
\mathbf{K}_k^\text{e}=
\mathbf{X}_k^\text{f}
\left(\mathbf{Y}_k^\text{f}\right)^\top
\left(
\mathbf{Y}_k^\text{f}
\left(\mathbf{Y}_k^\text{f}\right)^\top
+
\mathbf{E}_k^\text{o} \left(\mathbf{E}_k^\text{o}\right)^\top
\right)^{-1}
\end{equation}
where $\mathbf{Y}_k^\text{f}=\mathbf{H}_k\mathbf{X}_k^\text{f}$.

%Interestingly, it can be shown that the computation of the tangent linear operator $\mathbf{H}_k$ can be avoided. The details can be found in \cite[][Sec.~6.3.3]{Asch2016_SIAM}.  

Applications of EnKF strategies in fluid mechanics and engineering deal with a number of different topics such as wildfire propagation \cite{Rochoux2014_nhess}, combustion \cite{Labahn2019_pci}, turbulence modeling \cite{Xiao2016_jcp,Zhang2020_cf,Zhang2021_cf} and hybrid variational-EnKF methods \cite{Mons2019_jcp}. 
The state estimation procedure can be extended to infer the values of free parameters $\theta$ which describe the model. Several proposals have been reported in the literature (see the review work by Asch et al. \cite{Asch2016_SIAM} for an extended discussion). The strategy selected for this work is the \textit{dual estimation} proposed by Moradkhani et al. \cite{DENKF_MORADKHANI2005}. 

\subsection{Multigrid Ensemble Kalman Filter (MGEnKF)}

While the ensemble approximation $\mathbf{P}^\text{e}$ of the error covariance matrix $\mathbf{P}$ provides a significant reduction of the computational resources required by the Kalman filter, the generation of a database of $40-100$ elements may still be out of reach for complex applications in fluid mechanics. For this reason, the team has developed a multigrid ensemble Kalman filter (MGEnKF) \cite{Moldovan2021_jcp} strategy which exploits the numerical features of multigrid solvers. The algorithm is flexible and can be applied to numerical solvers using multiple refinement levels. Here, for sake of simplicity, it is illustrated on the classical two-grid FAS (Full Approximation Scheme) \cite{Brandt1977_mc,Wesseling1999_jcam} algorithm. This scheme employs a fine grid (solutions indicated with the superscript F) and a coarse grid (superscript C) in a three-step procedure: \lc{je ne reconnais pas en comparant avec l'article précédent cet algorithme}

\begin{enumerate}
\item A time advancement is performed starting from the solution $\mathbf{x}^\text{\tiny F}_{k-1}$ to obtain the state $(\mathbf{x}^\text{\tiny F}_{k})^{*}$
\item $(\mathbf{x}^\text{\tiny F}_{k})^{*}$ is projected on the coarse grid level and the state $\left(\mathbf{x}^\text{\tiny C}_k\right)^{*}=
\Pi_\text{\tiny C}\left(\left(\mathbf{x}_k^\text{\tiny F}\right)^{*}\right)
$ is obtained. Iterative calculations are used to filter out high-frequency noise and derive the solution $\left(\mathbf{x}^\text{\tiny C}_k\right)^{'}$
\item The difference between $\left(\mathbf{x}^\text{\tiny C}_k\right)^{'}$ and $\left(\mathbf{x}^\text{\tiny C}_k\right)^{*}$ is projected on the fine grid and the state $(\mathbf{x}^\text{\tiny F}_{k-1})^{*} + \Pi_\text{\tiny C}\left(\left(\mathbf{x}_k^\text{\tiny F}\right)^{'}-\left(\mathbf{x}_k^\text{\tiny F}\right)^{*}\right)$ is used as initial condition for a last set of iterations on the fine grid, which produces the final state $\mathbf{x}^\text{\tiny F}_{k}$
\end{enumerate}

\begin{figure}[htbp]

\includegraphics[width=0.95\textwidth]{figures/schema_MGENKF.pdf}
\caption{\label{fig:schema_MGENKF}
Schematic representation of the Multigrid Ensemble Kalman Filter (MGEnKF) \cite{Moldovan2021_jcp}. Two different levels of representation (fine and coarse grids) are used to obtain an estimation for the main simulation running on the fine grid. The inner and outer loop of the Dual Ensemble Kalman filter procedure are solved using ensemble members generated on the coarse grid.}
\end{figure}

\begin{figure}[htbp]

\includegraphics[width=1\textwidth]{figures/schema_inner_outer_loop.pdf}
\caption{\label{fig:schema_inou_loop}
Schematic representation of the box \textit{Dual EnKF} in Fig.~\ref{fig:schema_MGENKF}. Two optimization procedures, referred to as \textit{inner loop} and \textit{outer loop}, are sequentially performed.}
\end{figure}

A two-level EnKF, shown in Fig.~\ref{fig:schema_MGENKF}, is naturally integrated in the multigrid structure of the algorithm. This reduces the computational costs of the data assimilation procedure and contributes to render the solutions compatible with the dynamic equations of the model \cite{Moldovan2021_jcp}. 
The \textit{Dual EnKF} box shown in Fig.~\ref{fig:schema_MGENKF} consists of two distinct parts: an \textit{outer loop}, where observations are obtained from an external source of information, and an \textit{inner loop}, where fine grid solutions projected onto the coarse grid are used as surrogate observations. The complete general algorithm for MGEnKF is structured in the following operations:

\begin{enumerate}
\item \textbf{Predictor step}. The initial solution on the fine grid $\left(\mathbf{x}^\text{\tiny F}_{k-1}\right)^\text{a}$ is used to calculate a forecast state $\left(\mathbf{x}^\text{\tiny F}_{k}\right)^\text{f}$ 
$$
	\left(\mathbf{x}_k^\text{\tiny F}\right)^\text{f}=
	\mathbf{\mathcal{M}}^\text{\tiny F}_{k:k-1}\left(
	\left(\mathbf{x}_{k-1}^\text{\tiny F}\right)^\text{a},
	\overline{\mathbf{\theta}_{k}^\text{a}}\right)
$$ 
where $\mathbf{\mathcal{M}}^\text{\tiny F}_{k:k-1}$ is the model used on the fine grid and $\overline{\mathbf{\theta}_{k}^\text{a}}$ is a set of free parameters describing the setup of the model on the fine grid. Each member $i$ of the ensemble calculated on the coarse grid is also advanced in time
$$
	\left(\mathbf{x}_k^\text{\tiny C}\right)^\text{f,(i)}=
	\mathbf{\mathcal{M}}^\text{\tiny C}_{k:k-1}\left(
	\left(\mathbf{x}_{k-1}^\text{\tiny C}\right)^\text{a,(i)},
	\mathbf{\theta}_{k}^\text{f,(i)}\right) + \mathbf{\mathcal{C}}_{k:k-1}\left(
	\left(\mathbf{x}_{k-1}^\text{\tiny C}\right)^\text{a,(i)},
	\mathbf{\psi}_{k}^\text{f,(i)}\right),
$$ 
where $\mathbf{\mathcal{M}}^\text{\tiny C}_{k:k-1}$ is the coarse grid model parameterized by $\mathbf{\theta}_{k}^\text{f,(i)}$, while $\mathbf{\mathcal{C}}_{k:k-1}$ is an additional correction term included to compensate the loss of resolution due to calculations on the coarse grid \cite{Brajard2020_arxiv}. This additional model, whose structure is usually unknown, is driven by the set of free parameters $\mathbf{\psi}_{k}^\text{f,(i)}$.
%
\item \textbf{Projection on the coarse grid \& \textit{inner} loop}. $\left(\mathbf{x}^\text{\tiny F}_{k}\right)^\text{f}$ is projected on the coarse grid space via a projection operator $\Pi_\text{\tiny C}$, so that $\left(\mathbf{x}^\text{\tiny C}_{k}\right)^{*}$ is obtained, \textit{i.e.} 
$$
\left(\mathbf{x}^\text{\tiny C}_k\right)^{*}=
\Pi_\text{\tiny C}\left(\left(\mathbf{x}_k^\text{\tiny F}\right)^\text{f}\right)
$$
%
In this step, the flow field obtained on the fine mesh level is sampled to a set of observations $\left(\mathbf{y}_k^\text{\tiny C}\right)^\text{SO}=\left(\mathcal{H}_k^\text{\tiny C}\right)^\text{SO}\left(\mathbf{x}^\text{\tiny C}_k\right)^{*}$ which are used in the \textit{inner} loop as surrogate observations. Here, the EnKF is used as a \textit{parameter estimation only} scheme, \textit{i.e.} the ensemble states $\left(\mathbf{x}_k^\text{\tiny C}\right)^\text{f,(i)}$ are not modified, but the free parameters $\mathbf{\psi}_{k}^\text{f,(i)}$ are optimized to obtain values $\mathbf{\psi}_{k}^\text{a,(i)}$. This optimization targets an improvement of the prediction of the ensemble members simulated on the coarse grid via an update of the term $\mathbf{\mathcal{C}}_{k:k-1}\left(
	\left(\mathbf{x}_{k-1}^\text{\tiny C}\right)^\text{a,(i)},
	\mathbf{\psi}_{k}^\text{a,(i)}\right)$.
%
\item \textbf{\textit{Outer} loop}. If external observation $\left(\mathbf{y}_k^\text{\tiny C}\right)^\text{o}$ is available, the ensemble forecast $\left(\mathbf{x}^\text{\tiny C}_{k}\right)^{\text{f},(i)}$ is corrected with the standard Dual EnKF procedure to obtain $\left(\mathbf{x}^\text{\tiny C}_{k}\right)^{\text{a},(i)}$ as well as an update for the parameters $\mathbf{\theta}_{k}^{\text{a},(i)}$. %In this case clearly $\mathbf{\theta}_{k+1}^{\text{f},(i)}=\mathbf{\theta}_{k}^{\text{a},(i)}$, otherwise if observation is not available at the current time step $\mathbf{\theta}_{k}^{\text{a},(i)}$ is not modified.
%
\item \textbf{Determination of the state variables on the coarse grid}. 
In this step, the physical state of the main simulation is updated on the coarse grid. This solution, which will be referred to as $\left(\mathbf{x}^\text{\tiny C}_k\right)^{'}$, is obtained by classical iterative procedures on the coarse grid using the initial solution $\left(\mathbf{x}^\text{\tiny C}_{k}\right)^{*}$ if observations are not available. 
On the other hand, if observations are available, the Kalman gain matrix $\left(\mathbf{K}_k^\text{\tiny C}\right)^{x,\text{e}}$ determined in the framework of EnKF for the ensemble members is used to determine the coarse grid solution $\left(\mathbf{x}^\text{\tiny C}_k\right)^{'}$ through a KF operation, \textit{i.e.} 
		\begin{align*}
\left(\mathbf{x}^\text{\tiny C}_k\right)^{'} & =
\left(\mathbf{x}^\text{\tiny C}_k\right)^{*}+
\left(\mathbf{K}_k^\text{\tiny C}\right)^{x,\text{e}}
\left[
\left(\mathbf{y}_k^\text{\tiny C}\right)^\text{o}-
\left(\mathbf{\mathcal{H}}_k^\text{\tiny C}\right)^\text{o}
\left(\left(\mathbf{x}_k^\text{\tiny C}\right)^{*}\right)
\right]
		\end{align*} 
%
\item \textbf{Final iteration on the fine grid}. The fine grid state solution $\left(\mathbf{x}^\text{\tiny F}_k\right)^{'}$ is determined using the results obtained on the coarse space: $\left(\mathbf{x}^\text{\tiny F}_k\right)^{'}=\left(\mathbf{x}^\text{\tiny F}_{k}\right)^\text{f}+\Pi_\text{\tiny F}\left(\left(\mathbf{x}^\text{\tiny C}_k\right)^{'}-\left(\mathbf{x}^\text{\tiny C}_{k}\right)^{*}\right)$. The state $\left(\mathbf{x}^\text{\tiny F}_k\right)^\text{a}$ is obtained from a final iterative procedure starting from $\left(\mathbf{x}^\text{\tiny F}_k\right)^{'}$. 
\end{enumerate}

A detailed representation of the \textit{Dual EnKF} box shown in Fig.~\ref{fig:schema_MGENKF} is provided in Fig.~\ref{fig:schema_inou_loop}. This method is reminiscent of multilevel \cite{Hoel2016_SIAM,Siripatana2019_cg,KodyLaw2020,Fossum2020_cg} and multifidelity \cite{Gorodetsky2020_jcp,Popov2021_SIAM} ensemble techniques for data assimilation. However, this strategy does not need to include control variates as most approaches using stochastic Monte-Carlo sampling do. Therefore, only one main simulation on the fine grid is needed, significantly reducing the computational cost associated to the whole procedure.



==> Sec3-before_cordier.tex <==
\section{Optimization of numerical schemes on a coarse mesh}
\label{sec:apriorianalysis}

During time integration of solutions in the MGEnKF algorithm, classical numerical schemes unavoidably lead to  diffusive and dispersive errors that can excessively alter the representativity of solutions on too coarse meshes. It may inhibit their utilization for evaluating accurately the error covariance matrix required for updating the solution on the fine mesh.
An original feature of the present  MGEnKF algorithm presented in Sec.~\ref{sec:maths} is that the main solution advanced at the most refined level of the grid can also be used as surrogate observation to optimize the parameters of the numerical schemes used to advance the solutions on such coarse meshes. The principles guiding the choice of the numerical scheme and associated parametrization retained to control these numerical errors on coarse meshes are presented in this section.
Let us consider the prototype 1D linear advection equation of a scalar $u$ advected with advection velocity $c$.
\begin{equation}
\label{eq:1D_adv}
\frac{\partial u}{\partial t}+c \frac{\partial u}{\partial x}=0
\end{equation}

For the sake of clarity and conciseness, the discussion is restricted here to the discretization of this advection equation with explicit finite difference schemes on four-point stencils (second or third order accurate) for the case $c>0$ on a Cartesian mesh with a constant mesh size $\Delta x$.  The following considerations can quite easily be extended to non-linear systems with time and space varying advection velocity, irregular mesh or higher-order schemes. $\Delta t$ is the time step and  $\sigma=c\Delta t / \Delta x$ the CFL number.  $u_\text{j}^\text{k}$ represents the discrete numerical solution at the spatial location $x_\text{j}=(j-1)\Delta x$ at time $t=k\Delta t$.

A general one-parameter family of second order accurate schemes (see for example \cite{Hirsch2007} p. 364) may be defined on a backward upwind stencil $(j-2,j-1,j,j+1)$  as: 
\small
\begin{equation}
\label{eqschema}
\begin{aligned}
u_\text{j}^\text{k} & = & u_\text{j}^\text{k-1}-\frac{\sigma}{2} \left( u_\text{j+1}^\text{k-1}-u_\text{j-1}^\text{k-1} \right) +
\frac{\sigma^2}{2} \left( u_\text{j+1}^\text{k-1}-2 u_\text{j}^\text{k-1}+u_\text{j-1}^\text{k-1} \right) \\
& & +
\delta \left( -u_\text{j-2}^\text{k-1}+3u_\text{j-1}^\text{k-1}-3u_\text{j}^\text{k-1}+u_\text{j+1}^\text{k-1} \right)
\end{aligned}
\end{equation}

The terms in first line of equation \eqref{eqschema}  (remaining for $\delta=0$) correspond to the standard centered Lax Wendroff scheme. The last term in the second line (pre-multiplied by $\delta$) corresponds to a correction consistent with a dispersion term of the form $\delta \Delta x^3 u_{xxx}$ discretized on the extended backward upwind stencil.
This scheme is compatible with the linear advection equation \eqref{eq:1D_adv} with precision order proportional to $(\Delta x^2, \Delta t^2)$. If one retains the two first dominant error terms in the combination of Taylor expansions corresponding to these discrete terms forming scheme Eq \ref{eqschema}, the following equivalent differential equation is obtained:
\begin{equation}
\label{eqequiv}
\begin{aligned}
\frac{\partial u}{\partial t}+c \frac{\partial u}{\partial x} & = & \frac{c}{6} \left[ 6\delta -
\sigma \left( 1-\sigma^2\right)\right] \Delta_x^2 \frac{\partial ^3 u}{\partial x^3} \\
 & & - \frac{c}{8} \left[ \delta \left( 1-2 \sigma \right) + \frac{\sigma^2}{4} \left( 1 - \sigma^2 \right)  \right]  \Delta_x^3 \frac{\partial ^4 u}{\partial x^4} \\
\end{aligned}
\end{equation}
  
For arbitrary values of $\delta$, Eq. \eqref{eqequiv} shows that the dominant numerical error of scheme \eqref{eqschema} is of dispersive nature with an error proportional to $\Delta x^2$ and a less dominant (third-order) diffusive error term. Their expressions already show that their relative level varies both as function of $\sigma$ and $\delta$. It does not seem interesting to optimize a priori the choice of $\sigma$, in order keep the MGEnKF algorithm sufficiently flexible and general. Therefore, it is chosen to target an optimization for $\delta$ only with a strategy suitable for any value of $\sigma$. This choice allows the user to set the value of $\sigma$ based on practical constraints, such as for synchronizing simulations with observation data available.
The level of this error can then be partially controlled through the parameter $\delta$ for a given $\sigma$. By setting in particular $\delta = \sigma(1-\sigma^2)/6$, this dominant error term cancels out and the scheme becomes third order accurate in space with now a dominant error term of diffusive nature proportional to $\Delta x^3$. Different values for $\delta$ maintain the formal second order accuracy but can induce significantly different effective evolution of the numerical errors. An illustration of this possible error behavior (and thus potential a priori control) is shown in Fig \ref{fig:figerror}. These errors are here quantified through a classical Fourier analysis, through which the expression of the complex gain factor $G = Re(G) + i \, Im(G)$ is extracted as function of the phase angle $\phi = m \Delta x$ with $m$ corresponding to a spatial wavenumber. It is worth recalling that the phase angle $\phi=m \Delta x = 2\pi / \lambda$, where $\lambda$ is the spatial wavelength, can also be written as $\phi = 2\pi / (N-1)$, where N represents the number of points used to discretize the signal over $\lambda$. The modulus of the gain factor $|G|$ should remain less than 1 for the whole range of $\phi$ present in the signal being advected to ensure stability. However, $1-|G|$ represents the level of numerical diffusion and might be minimized to avoid artificial decrease of wave amplitude components. The dispersive error is here characterized by $\epsilon_{\phi} =  atan(-Im(G)/Re(G)) / \sigma \phi $, which corresponds to the spurious multiplicative factor affecting the expected phase velocity of wave components. A good numerical scheme should control it to remain as close as possible to the unity value to limit phase advance or delay observed for $\epsilon_{\phi}>1$ or $\epsilon_{\phi}<1$, respectively. In Fig. \ref{fig:figerror}, the scheme responses for various $\delta$ as function of $\phi$ and $\sigma$ show how different functional evolutions of $\delta$ may thus lead to significantly different effective error properties. 
The case $\delta=0$ (Lax Wendroff scheme) is characterized by a dominant phase lag within the stability bounds $0<\sigma<1$. The choice $\delta=\sigma (1-\sigma)/2$ (not shown) corresponds to  Beam and Warming scheme which yields a dominant phase advance error for the similar range of variation of $0<\sigma<1$. The case $\delta = \sigma (1-\sigma)/4$ corresponds to the famous Fromm's scheme which compensates to some extent the delay and advance phase errors of the two aforementioned schemes for a wide range of $\sigma$. It can be indeed noticed in Fig. \ref{fig:figerror} that isolines of $\epsilon_{\phi}$ for values lower than one are significantly shifted towards the higher values of $\phi$, indicating that dispersive error levels can be a priori significantly reduced in the intermediate range of $\phi$ corresponding to practical simulation cases. However, the reduction of diffusive error, as illustrated with $|G|$ is far less efficient, in particular for high values of $\sigma$. This diffusive error is even seen to increase on the contrary for lower values of $\sigma$ and high values of $\phi$. 

It should be kept in mind that the MGEnKF algorithm employs ensemble members which has to be generated using relatively coarse grids (thus high values of $\phi$ for a given signal to advect) for which both the dispersive and diffusive terms are likely to be important. Both Eq. \ref{eqequiv} and these aforementioned observations of the non-monotonic and uncorrelated evolutions of $|G|$ and $\epsilon_{\phi}$ suggest accordingly that adjusting only this single parameter $\delta$ is not sufficient to allow a satisfactory control of both kind of error at the same time. An optimization of $\delta$ to reduce the dispersive error may indeed lead to deteriorate the diffusive behavior of the scheme. This justifies a first important choice retained for the present optimization strategy, which consists in considering also an additional correction to scheme \eqref{eqschema} for the present optimization, with the same order as the dispersive correction term in factor of $\delta$. This term is chosen as being consistent with $\alpha \Delta x^2 \frac{\sigma^2}{2}\frac{\partial ^2 u}{\partial x^2}$. With negative values of $\alpha$, this term will be expected to add an anti-diffusive behavior, counteracting the diffusion error intrinsically associated with scheme \eqref{eqschema}. The combined use of both correction terms is thus expected to allow a more relevant separated control of both dispersion and diffusion errors.


\begin{figure}[htbp]
\centering
\includegraphics[width=0.8\textwidth, trim=0cm 0cm 0cm 0cm,clip]{figures/errorLWvsFromm.png}
\caption{\label{fig:figerror} Comparison of diffusive (top) and dispersive (bottom) errors for two different a priori parametrizations of $\delta$.}
\end{figure} 

As previously observed in Fig. \ref{fig:figerror}, the effective scheme response significantly varies as function of $\phi$.
For a given value of $\sigma$ and a given mesh size, an optimization of $\delta$ and $\alpha$, considered as constant parameters, could indeed only allow a significant reduction of numerical error in a relatively limited range of $\phi$ (thus enabling a control of accuracy for representing a limited range of the spectral content associated to the signal to advect). In view of considering complex (spectrally richer) solutions and extending the use of this scheme to non-linear models, possibly leading to spatially evolving frequency content, it is thus also chosen to consider spatially varying functions for $\delta$ and $\alpha$ instead of constant values. This variability, which will be represented expressing the parameters via spatial expansions of polynomials, will allow for local numerical optimization on coarse meshes.
 
\paragraph{Summary: numerical model retained to perform coarse-grid simulations}~\\
Following the previous a priori analysis given all along this section, the following numerical scheme is finally retained:
\begin{equation}
\label{eq:1D_adv_oneparameter_parametrized}
\begin{aligned}
u_\text{j}^\text{k} & = & u_\text{j}^\text{k-1}-\frac{\sigma}{2} \left( u_\text{j+1}^\text{k-1}-u_\text{j-1}^\text{k-1} \right) +
\left(1+\alpha\right)\frac{\sigma^2}{2} \left( u_\text{j+1}^\text{k-1}-2 u_\text{j}^\text{k-1}+u_\text{j-1}^\text{k-1} \right) \\
& & +\left(\delta+\gamma\right) \left( -u_\text{j-2}^\text{k-1}+3u_\text{j-1}^\text{k-1}-3u_\text{j}^\text{k-1}+u_\text{j+1}^\text{k-1} \right) \\
& = &	\mathbf{\mathcal{M}}_{k:k-1}\left(u, \sigma, \delta \right) + \mathbf{\mathcal{C}}_{k:k-1}\left( u, \sigma, \alpha, \gamma \right) 
\end{aligned}
\end{equation}
Here, one can see that the optimization of $\delta$ is not performed directly, but via a parameter $\gamma$ which measures the deviation of the optimized dispersion coefficient from the constant value $\delta= \sigma(1-\sigma^2)/4$ proposed by Fromm. This choice has been performed to provide a clear separation between the dynamic model $\mathbf{\mathcal{M}}$ and the correction model $\mathbf{\mathcal{C}}$ when comparing Eq.~\ref{eqschema} and Eq.~\ref{eq:1D_adv_oneparameter_parametrized}. The variability in space of the coefficients $\gamma(x)$ and $\alpha(x)$ is obtained expressing them in terms of a Legendre Polynomial expansion (truncated to the order $n$):

 \begin{equation}
 \gamma\left(x\right)=\gamma_\text{0}P_\text{0}\left(x\right)+\gamma_\text{1}P_\text{1}\left(x\right)...+\gamma_\text{n}P_\text{n}\left(x\right)\label{eq:beta_legendre},
\end{equation}

\begin{equation}
\alpha\left(x\right)=\alpha_\text{0}P_\text{0}\left(x\right)+\alpha_\text{1}P_\text{1}\left(x\right)...+\alpha_\text{n}P_\text{n}\left(x\right)\label{eq:alpha_legendre}.
\end{equation}

%$P_\text{n}$ is here the higher-order Legendre Polynomial after which a trucation of the series is perfrepresenting the truncation order. An n-order accurate approximation of $\gamma$ and $\alpha$ requires $n+1$ coefficients.
Preliminary tests showed that $4$-th order representation ($n=4$) is satisfactory for the tests considered in the present study. The inner loop will be used to optimize the expansion coefficients for a total of $10$ parameters (five expansion coefficients $\gamma_i$ and five expansion coefficients $\alpha_i$). The values for these parameters could possibly be constrained during the inner loop optimization in order to accept only values leading to stable solutions. In particular, the extended stability constraint for the present scheme in absence of additional anti-diffusive correction is imposed, which reads as:
\begin{equation}
\label{stab}
\gamma (1-2\sigma) + \frac{1}{4} \sigma^2 (1-\sigma^2) \geq 0
\end{equation}

%The \textit{inner loop} will perform an internal optimization of these model correction terms, satisfying such stability constraints while improving the accuracy of the model used on coarse meshes.


==> Sec3-lo.tex <==
\section{Optimization of numerical integration schemes on a coarse mesh}
\label{sec:apriorianalysis}

%During time integration of solutions in the MGEnKF algorithm, 
Numerical schemes unavoidably lead to  diffusive and dispersive errors that can excessively alter the representativity of solutions on too coarse meshes. 
These errors can lead to an imprecise determination of the error covariance matrix, prohibiting the updating of the solution on the fine mesh.
An original feature of the MGEnKF algorithm presented in Sec.~\ref{sec:maths} is that the solution advanced at the most refined level of the grid can also be used as surrogate observation to optimize the parameters of the numerical schemes. 
In this section, we present the principles guiding the choice of the numerical scheme and associated parametrization retained to control the numerical errors on coarse meshes.
Let us consider the prototype 1D linear advection equation of a scalar quantity $u$ advected with the constant velocity $c$:
\begin{equation}
\label{eq:1D_adv}
\frac{\partial u}{\partial t}+c \frac{\partial u}{\partial x}=0
\end{equation}

For simplicity of presentation, we restrict ourselves to using an explicit finite difference scheme on four-point stencils (second or third order accurate) for the case $c>0$.
The spatial discretization is performed on a Cartesian mesh with a constant size $\Delta x$.
$\Delta t$ is the time step and  $\sigma=c\Delta t / \Delta x$ the CFL number.  $u_\text{j}^\text{k}$ represents the discrete numerical solution at the spatial location $x_\text{j}=(j-1)\Delta x$ at time $t=k\Delta t$.
The following considerations can be extended quite easily to non-linear systems with time and space varying advection velocity, irregular mesh or higher-order schemes. 

A general one-parameter family of second order accurate schemes (see for example \cite{Hirsch2007} p. 364) may be defined on a backward upwind stencil $(j-2,j-1,j,j+1)$  as: 
\begin{equation}
\label{eqschema}
\begin{aligned}
u_\text{j}^\text{k} & = & u_\text{j}^\text{k-1}-\frac{\sigma}{2} \left( u_\text{j+1}^\text{k-1}-u_\text{j-1}^\text{k-1} \right) +
\frac{\sigma^2}{2} \left( u_\text{j+1}^\text{k-1}-2 u_\text{j}^\text{k-1}+u_\text{j-1}^\text{k-1} \right) \\
& & +
\delta \left( -u_\text{j-2}^\text{k-1}+3u_\text{j-1}^\text{k-1}-3u_\text{j}^\text{k-1}+u_\text{j+1}^\text{k-1} \right)
\end{aligned}
\end{equation}

The first line of \eqref{eqschema} corresponds to the standard centered Lax Wendroff scheme. The second line can be interpreted as the discretization of an additional dispersion term of the form $\delta \Delta x^3 u_{xxx}$.
The expression \eqref{eqschema} is compatible with the linear advection equation \eqref{eq:1D_adv} discretized at precision order proportional to $(\Delta x^2, \Delta t^2)$. If one retains the two first dominant error terms in the combination of Taylor expansions corresponding to these discrete terms forming scheme \eqref{eqschema}, \lc{comprends pas cette phrase} the following equivalent differential equation is obtained:
\begin{equation}
\label{eqequiv}
\begin{aligned}
\frac{\partial u}{\partial t}+c \frac{\partial u}{\partial x} & = & \frac{c}{6} \left[ 6\delta -
\sigma \left( 1-\sigma^2\right)\right] \Delta_x^2 \frac{\partial ^3 u}{\partial x^3} & \\
 & & - \frac{c}{8} \left[ \delta \left( 1-2 \sigma \right) + \frac{\sigma^2}{4} \left( 1 - \sigma^2 \right)  \right]  \Delta_x^3 \frac{\partial ^4 u}{\partial x^4} & + \mathcal{O}\left(\Delta_x^4\right)\\
\end{aligned}
\end{equation}
  
Equation \eqref{eqequiv} reveals that the dominant numerical error of \eqref{eqschema} is dispersive with an error proportional to $\Delta x^2$ and that a less dominant (third-order) diffusive error term occurs. The expressions of these errors show that their relative level varies both as function of $\sigma$ and $\delta$. 
In order to keep the MGEnKF algorithm sufficiently flexible and general, we will not search to optimize the parameter $\sigma$.
Therefore, it is chosen to target only an optimization for $\delta$  with a strategy suitable for any value of $\sigma$. This choice allows the user to set the value of $\sigma$ based on practical constraints, such as for synchronizing simulations with available observation data.
The level of the dominant error can be controlled through the parameter $\delta$. By setting in particular $\delta = \sigma(1-\sigma^2)/6$, the dominant error term cancels out and the scheme becomes third order accurate in space with now a  diffusive dominant error term proportional to $\Delta x^3$. Other values of $\delta$ maintain the formal second order accuracy but can induce significantly different effective evolution of the numerical errors. 
\begin{figure}[htbp]
\centering
%\includegraphics[width=0.8\textwidth, trim=0cm 0cm 0cm 0cm,clip]{figures/errorLWvsFromm.png}
\includegraphics[width=0.9\textwidth, trim=0cm 0cm 0cm 0cm,clip]{figures/errorLWvsFromm.pdf}
\caption{\label{fig:figerror} Comparison of diffusive ($\epsilon_D=|G|$, top) and dispersive ($\epsilon_{\phi}$, bottom) errors for two different a priori parametrizations of $\delta$. $\delta=0$ (left column) corresponds to the Lax Wendroff scheme and $\delta=\sigma\left(1-\sigma\right)/4$ (right column) to Fromm's scheme.}
\end{figure}
An illustration of this is shown in Fig. \ref{fig:figerror} where the diffusion and dispersion errors are represented. These errors are quantified through a classical Fourier analysis, through which the expression of the complex gain factor $G = \text{Re}(G) + \jmath \, \text{Im}(G)$ is extracted as function of the phase angle $\phi = m \Delta x$ with $m$ corresponding to a spatial wavenumber. It is worth recalling that the phase angle $\phi=m \Delta x = 2\pi / \lambda$, where $\lambda$ is the spatial wavelength, can also be written as $\phi = 2\pi / (N-1)$, where N represents the number of points used to discretize the signal over $\lambda$. 
To ensure stability, the modulus of the gain factor $|G|$ should remain less than 1 for the whole range of $\phi$ present in the signal being advected. 
As for him, $1-|G|$ represents the level of numerical diffusion.
This quantity might be minimized to avoid artificial decrease of wave amplitude components. The dispersive error is here characterized by $\epsilon_{\phi} =  \arctan(-\text{Im}(G)/\text{Re}(G)) / \sigma \phi $, which corresponds to the spurious multiplicative factor affecting the expected phase velocity of wave components. 
A good numerical scheme should keep the value of $\epsilon_{\phi}$ as close as possible to unity to limit phase advance or delay observed for $\epsilon_{\phi}>1$ or $\epsilon_{\phi}<1$, respectively. 
Figure \ref{fig:figerror} clearly shows the role played by $\delta$ on the diffusion and dispersion errors. 
The case $\delta=0$ (Lax Wendroff scheme) is characterized by a dominant phase lag within the stability bounds $0<\sigma<1$. The choice $\delta=\sigma (1-\sigma)/2$ (not shown) corresponds to  Beam and Warming scheme which yields a dominant phase advance error for $0<\sigma<1$. The case $\delta = \sigma (1-\sigma)/4$ corresponds to the famous Fromm's scheme which compensates to some extent the phase errors of the two aforementioned schemes for a wide range of $\sigma$. Indeed, we notice in Fig. \ref{fig:figerror} that isolines of $\epsilon_{\phi}$ lower than unity are significantly shifted towards the higher values of $\phi$, indicating that dispersive error levels can be a priori significantly reduced in the intermediate range of $\phi$ corresponding to practical simulation cases. However, the reduction of diffusive errors, as illustrated with $|G|$ is far less efficient, in particular for high values of $\sigma$. The diffusive errors are even seen to increase for lower values of $\sigma$ and high values of $\phi$. 

We have to keep in mind that the MGEnKF algorithm employs ensemble members which has to be generated using relatively coarse grids (thus high values of $\phi$) for which both the dispersive and diffusive errors are likely to be important. The aforementioned observations of the non-monotonic and uncorrelated evolutions of $|G|$ and $\epsilon_{\phi}$ suggest that adjusting only $\delta$ is not sufficient to allow a satisfactory control of both kind of errors at the same time. 
An optimization of $\delta$ made for reducing the dispersive error could undesirably deteriorate the diffusive behavior of the scheme. 
This justifies that in the optimization strategy that we consider in Sec.~\ref{sec:advection}, we add to \eqref{eqschema} an additional correction of the same order as the dispersive correction term in factor of $\delta$. 
This correction is chosen as being consistent with $\alpha \Delta x^2 \dfrac{\sigma^2}{2}\dfrac{\partial ^2 u}{\partial x^2}$. With negative values of $\alpha$, this term will be expected to add an anti-diffusive behavior, counteracting the diffusion error intrinsically associated with the scheme \eqref{eqschema}. The combined use of both correction terms is thus expected to allow a more relevant separated control of both dispersion and diffusion errors.

As previously observed in Fig. \ref{fig:figerror}, the properties of the numerical scheme significantly vary as function of $\phi$.
It is therefore far from being evident that considering $\delta$ and $\alpha$ as constant optimization parameters is sufficient to reduce the numerical error over a wide range of $\phi$ scales. 
In view of considering complex (spectrally richer) solutions and extending the use of this scheme to non-linear models, possibly leading to spatially evolving frequency content, it is thus also chosen to consider spatially varying functions for $\delta$ and $\alpha$ instead of constant values. This variability, which will be represented by expressing these parameters via spatial expansions of polynomials, will allow for local numerical optimization on coarse meshes.
 
\paragraph{Summary: numerical scheme retained to perform coarse-grid simulations}~\\
Following the a priori analysis given all along this section, the following numerical scheme is finally retained:
\begin{equation}
\label{eq:1D_adv_oneparameter_parametrized}
\begin{aligned}
u_\text{j}^\text{k} & = & u_\text{j}^\text{k-1}-\frac{\sigma}{2} \left( u_\text{j+1}^\text{k-1}-u_\text{j-1}^\text{k-1} \right) +
\left(1+\alpha\right)\frac{\sigma^2}{2} \left( u_\text{j+1}^\text{k-1}-2 u_\text{j}^\text{k-1}+u_\text{j-1}^\text{k-1} \right) \\
& & +\underbrace{\left(\delta_\text{F}+\gamma\right)}_{\delta} \left( -u_\text{j-2}^\text{k-1}+3u_\text{j-1}^\text{k-1}-3u_\text{j}^\text{k-1}+u_\text{j+1}^\text{k-1} \right) \\
& = &	\mathbf{\mathcal{M}}_{k:k-1}\left(u;\sigma, \delta_\text{F} \right) + \mathbf{\mathcal{C}}_{k:k-1}\left( u;\sigma, \alpha, \gamma \right) 
\end{aligned}
\end{equation}
\lc{pour moi, il ne faudrait plus utiliser ici la variable delta car gamma, autant que je le comprenne, est introduit comme une variation par rapport à une valeur particulière de delta donnée par Fromm. Je choisis donc d'appeler cette valeur particulière de delta $\delta_\text{F}$.}
Here, one can see that the optimization of $\delta$ is not performed directly, but via a parameter $\gamma$ which measures the deviation of the optimized dispersion coefficient from the constant value $\delta_\text{F} \triangleq \sigma(1-\sigma^2)/4$ proposed by Fromm. This choice has been performed to provide a clear separation between the dynamical model $\mathbf{\mathcal{M}}$ and the correction model $\mathbf{\mathcal{C}}$ when comparing \eqref{eqschema} and \eqref{eq:1D_adv_oneparameter_parametrized}. The variability in space of the coefficients $\gamma$ and $\alpha$ is obtained expressing them in terms of Legendre Polynomial expansions truncated to the order $n$:
 \begin{equation}
 \gamma\left(x\right)=\gamma_\text{0}P_\text{0}\left(x\right)+\gamma_\text{1}P_\text{1}\left(x\right)+\cdots+\gamma_\text{n}P_\text{n}\left(x\right)\label{eq:beta_legendre},
\end{equation}
and
\begin{equation}
\alpha\left(x\right)=\alpha_\text{0}P_\text{0}\left(x\right)+\alpha_\text{1}P_\text{1}\left(x\right)+\cdots+\alpha_\text{n}P_\text{n}\left(x\right)\label{eq:alpha_legendre}.
\end{equation}

%$P_\text{n}$ is here the higher-order Legendre Polynomial after which a trucation of the series is perfrepresenting the truncation order. An n-order accurate approximation of $\gamma$ and $\alpha$ requires $n+1$ coefficients.
Preliminary tests showed that $4$-th order representation ($n=4$) is satisfactory for the cases considered in this study. The inner loop will be used to optimize the expansion coefficients for a total of $10$ parameters (five expansion coefficients $\gamma_i$ and five expansion coefficients $\alpha_i$). The values for these parameters could possibly be constrained during the inner loop optimization in order to accept only values leading to stable solutions. In particular, the extended stability constraint for the present scheme in absence of additional anti-diffusive correction is imposed, which reads as\lc{$\alpha$ ne joue aucun rôle dans cette condition?}:
\begin{equation}
\label{stab}
\gamma (1-2\sigma) + \frac{1}{4} \sigma^2 (1-\sigma^2) \geq 0
\end{equation}

%The \textit{inner loop} will perform an internal optimization of these model correction terms, satisfying such stability constraints while improving the accuracy of the model used on coarse meshes.

